Differentiable Factor Graph Optimization for Learning Smoothers

A recent line of work has shown that end-to-end optimization of Bayesian filters can be used to learn state estimators for systems whose underlying models are difficult to hand-design or tune, while retaining the core advantages of probabilistic state estimation. As an alternative approach for state estimation in these settings, we present an end-to-end approach for learning state estimators modeled as factor graph-based smoothers. By unrolling the optimizer we use for maximum a posteriori inference in these probabilistic graphical models, we can learn probabilistic system models in the full context of an overall state estimator, while also taking advantage of the distinct accuracy and runtime advantages that smoothers offer over recursive filters. We study this approach using two fundamental state estimation problems, object tracking and visual odometry, where we demonstrate a significant improvement over existing baselines. Our work comes with an extensive code release, which includes training and evaluation scripts, as well as Python libraries for Lie theory and factor graph optimization: https://sites.google.com/view/diffsmoothing/

==> 3-unused.tex <==





This section is unused








\section{State Estimation Background}

\by{Background section feels to long. Can cut or move some into ``approach''}

\subsection{State Estimation}
% In robotics, this kind of sensor fusion has been studied in the framework of state estimation for several decades.
% In these problems, our goal is to process incoming sensory inputs and use them to recover an estimate of system state.
In robotics, state estimation has primarily been studied under two frameworks:

\subsubsection{Filtering}
Most commonly, state estimators are built using a \textit{filtering} structure.
In a filter, we maintain a probabilistic belief about the current state of our system, which is then updated at each timestep with incoming sensory inputs.
This results in a process that requires approximations for non-linear systems, but is recursive in nature and only requires a constant amount of memory for problems with fixed state dimensionalities: the output at a given timestep $t$ can be computed from only (a) the output from $t - 1$ and (b) any inputs corresponding to timestep $t$.

\subsubsection{Smoothing}
In contrast to filtering, smoothing requires us to retain all past measurements and continuously recover full trajectories.
This approach may initially seem inefficient compared to filtering, but prior works have shown that they can outperform filtering approaches in terms of both accuracy and runtime \cite{dellaert2006squareroot,strasdat2012visual}.
One common way to represent and solve these problems, which we focus on in this project, is with a bipartite probabilistic graphical model called a factor graph. %; an example is provided in Figure \ref{fig:factor_graphs}.
We elaborate on factors graphs and discuss their advantages in Section \ref{sec:factor_graphs}.

\subsection{Factor Graph Optimization}
\label{sec:factor_graphs}

% While filtering-based state estimators are ubiquitous in practical robotics, their applications are restricted by practical limitations.
% To work around these constraints, many modern systems rely on \textit{smoothing} for state estimation, which can be faster, more robust, and more accurate \cite{strasdat2012visual}.
% While there are many ways to set up these smoothing problems, one common approach is by first representing them using a factor graph.
Factor graphs are a class of probabilistic graphical models that have demonstrated impressive versatility in real-world state estimation: by representing probabilistic functions as bipartite graphs connecting \textit{variables} to solve for and \textit{factors} that define conditional probabilities on these variables, these models provide highly general abstractions that have been applied to a wealth of problems in robotics.

Formally, each factor encodes a conditional probability density given by
\begin{equation}
    \bm{\phi}_i (X_i) \propto \exp(-\frac{1}{2} \lvert\lvert h_i(X_i) - z_i \rvert\rvert_{\Sigma_i}^2)
\end{equation}
which for Gaussian factors is computed using the Mahalanobis distance between an expected measurement $h_i(X_i)$ and a measurement vector $z_i$ given a measurement uncertainty $\Sigma_i$, where $X_i$ is a set of connected variables and $h_i$ is our measurement model.

After modeling estimation inputs as factors and outputs as variables, we can solve for our state estimates by performing maximum a posteriori inference.
With Gaussian noise assumptions, this reduces to a simple nonlinear optimization:
\begin{equation}
    \begin{split}
        X^*
        &= {\arg\max}_X \prod_i \bm{\phi}_i(X_i)\\
        &= {\arg\max}_X \prod_i \exp(-\frac{1}{2} \lvert\lvert h_i(X_i) \ominus z_i \rvert\rvert_{\Sigma_i}^2)\\
        &= {\arg\min}_X \sum \lvert\lvert h_i(X_i) - z_i \rvert\rvert_{\Sigma_i}^2\\
    \end{split}
\end{equation}

While applying this approach to state estimation requires solving a nonlinear optimization problem at each timestep, significant performance gains can be made because of the connection between the locality of a graph and the sparsity of its matrix representation \cite{dellaert2006squareroot}.
Real-time applications can also benefit from incremental updates to a matrix factorization \tocite{isam} or Bayes tree data structure \tocite{isam2}.
% An example smoothing problem drawn as a factor graph can be found in Figure \ref{fig:factor_graphs}.

% Not entirely sure where to put this, if anywhere
While our focus is on modeling state estimation problems as inference on factor graphs, the underlying algorithms are not inherently tied to this particular probabilistic graphical model. % and the terminology used to describe mathematically equivalent approaches vary in literature.
Mathematically equivalent optimization over sparse residuals also appears when visualizing these systems as hypergraphs \cite{kummerle2011g2o}, where factor nodes are replaced by hyperedges that can connect any number of variable nodes, and in application-specific algorithms for problems like pose graph optimization \cite{OlsonGraph2006} and bundle adjustment \cite{strasdat2012visual}.

